HIR-Diff: Unsupervised Hyperspectral Image Restoration Via Improved Diffusion Models

Hyperspectral image (HSI) restoration aims at recovering clean images from degraded observations and plays a vital role in downstream tasks. Existing model-based methods have limitations in accurately modeling the complex image characteristics with handcraft priors, and deep learning-based methods suffer from poor generalization ability. To alleviate these issues, this paper proposes an unsupervised HSI restoration framework with pre-trained diffusion model (HIR-Diff), which restores the clean HSIs from the product of two low-rank components, i.e., the reduced image and the coefficient matrix. Specifically, the reduced image, which has a low spectral dimension, lies in the image field and can be inferred from our improved diffusion model where a new guidance function with total variation (TV) prior is designed to ensure that the reduced image can be well sampled. The coefficient matrix can be effectively pre-estimated based on singular value decomposition (SVD) and rank-revealing QR (RRQR) factorization. Furthermore, a novel exponential noise schedule is proposed to accelerate the restoration process (about 5$\times$ acceleration for denoising) with little performance decrease. Extensive experimental results validate the superiority of our method in both performance and speed on a variety of HSI restoration tasks, including HSI denoising, noisy HSI super-resolution, and noisy HSI inpainting. The code is available at https://github.com/LiPang/HIRDiff.

==> sec/3_notations.tex <==
\section{Notations}
\label{sec:notations}
A scalar, a vector, a matrix, and a tensor are defined as $x, \mathbf{x}, \mathbf{X}, \mathcal{X}$ respectively. Given a third order tensor $\mathcal{X}\in\mathbb{R}^{M\times N\times B}$ and a matrix $\mathbf{E}\in\mathbb{R}^{B\times C}$, the mode-3 multiplication can be defined as
\begin{equation}\label{mode3multi}
(\mathcal{X}\times_3\mathbf{E})_{(m,n,b)}=\sum_{i=1}^C\mathcal{X}_{(m,n,i)}\mathbf{E}_{(b,i)}.
\end{equation}
$\mathbf{X}_{(3)} \in \mathbb{R}^{B\times MN}$ denotes the mode-3 unfolding of $\mathcal{X}$ and is obtained by flattening the first two dimensions of $\mathcal{X}$. And $\mathbf{fold}_3(\mathbf{X}_{(3)})$ means reshaping $\mathbf{X}_{(3)}$ back to $\mathcal{X}$. $\det(\mathbf{X})$ denotes the determinant value of $\mathbf{X}$. The L2-norm of $\mathbf{x} \in \mathbb{R}^{K}$ is denoted as $\| \mathbf{x} \|_2 = \sqrt{\sum_{i=1}^{K}x_i^2}$. $\|\mathcal{X}\|_F = \sqrt{\sum_{i,j,k}x_{i,j,k}^2}$ denotes the Frobenius norm of tensor $\mathcal{X}\in\mathbb{R}^{M\times N\times B}$.

